The extraordinary linear polarisation structure of the southern Centaurus A lobe revealed by ASKAP

We present observations of linear polarisation in the southern radio lobe of Centaurus A, conducted during commissioning of the Australian Square Kilometre Array Pathfinder (ASKAP) telescope. We used 16 antennas to observe a 30 square degree region in a single 12 hour pointing over a 240 MHz band centred on 913 MHz. Our observations achieve an angular resolution of $26\times33$ arcseconds (480 parsecs), a maximum recoverable angular scale of 30 arcminutes, and a full-band sensitivity of 85 $\muup$Jy beam$^{-1}$. The resulting maps of polarisation and Faraday rotation are amongst the most detailed ever made for radio lobes, with of order 10$^5$ resolution elements covering the source. We describe several as-yet unreported observational features of the lobe, including its detailed peak Faraday depth structure, and intricate networks of depolarised filaments. These results demonstrate the exciting capabilities of ASKAP for widefield radio polarimetry.

==> journals.tex <==
%-- Journal definitions for the bibliography
\def\latex{\LaTeX{}}
\def\azh{Astronomicheskii Zhurnal}                   % Astronomicheskii Zhurnal
\def\aj{AJ}                   % Astronomical Journal
\def\araa{ARA\&A}             % Annual Review of Astron and Astrophys
\def\apj{ApJ}                 % Astrophysical Journal
\def\apjl{ApJL}                % Astrophysical Journal, Letters
\def\apjs{ApJS}               % Astrophysical Journal, Supplement
\def\apss{Ap\&SS}             % Astrophysics and Space Science
\def\aap{A\&A}                % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}              % Astronomy and Astrophysics, Supplement
\def\mnras{MNRAS}             % Monthly Notices of the RAS
\def\nat{Nature}              % Nature
\def\pasp{PASP}               % Publications of the ASP
\def\pasa{PASA}
\def\pasj{PASJ} %Publications of the Astronomical Society of Japan
\def\nar{NewAR}
\def\procspie{Proc. SPIE.}
\def\skytel{Sky \& Telescope}              % Sky \& Telescope
\def\ssr{Space Sci. Rev.}  %Space science reviews
\def\iaucirc{IAU circ.}

